Fully probabilistic quasar continua predictions near Lyman-{\alpha} with conditional neural spline flows

Measurement of the red damping wing of neutral hydrogen in quasar spectra provides a probe of the epoch of reionization in the early Universe. Such quantification requires precise and unbiased estimates of the intrinsic continua near Lyman-$\alpha$ (Ly$\alpha$), a challenging task given the highly variable Ly$\alpha$ emission profiles of quasars. Here, we introduce a fully probabilistic approach to intrinsic continua prediction. We frame the problem as a conditional density estimation task and explicitly model the distribution over plausible blue-side continua ($1190\ \unicode{xC5} \leq \lambda_{\text{rest}} < 1290\ \unicode{xC5}$) conditional on the red-side spectrum ($1290\ \unicode{xC5} \leq \lambda_{\text{rest}} < 2900\ \unicode{xC5}$) using normalizing flows. Our approach achieves state-of-the-art precision and accuracy, allows for sampling one thousand plausible continua in less than a tenth of a second, and can natively provide confidence intervals on the blue-side continua via Monte Carlo sampling. We measure the damping wing effect in two $z>7$ quasars and estimate the volume-averaged neutral fraction of hydrogen from each, finding $\bar{x}_\text{HI}=0.304 \pm 0.042$ for ULAS J1120+0641 ($z=7.09$) and $\bar{x}_\text{HI}=0.384 \pm 0.133$ for ULAS J1342+0928 ($z=7.54$).

==> captions/ULASJ1120+0641.tex <==
\begin{figure*}
	\includegraphics[width=\textwidth]{figures/ULASJ1120+0641_tight.png}
    \caption{The observed spectrum of ULAS J1120+0641 ($z=7.09$) in grey overlaid with its smoothed continuum estimate in red and our prediction of its underlying intrinsic continuum in blue accompanied by 1-sigma (68\%) and 2-sigma (95\%) confidence intervals.}
    \label{fig:ULASJ1120+0641}
\end{figure*}

==> captions/ULASJ1120+0641_comp.tex <==
\begin{figure}
	\includegraphics[width=\columnwidth]{figures/ULASJ1120+0641_comp_tight_rev1.png}
    \caption{\spectre's prediction of ULAS J1120+0641's intrinsic blue-side spectrum compared with previous predictions by \citet{qsanndra}, \citet{daviesPCA},  \citet{greigLya}, and \citet{J1120}. The neural network models, \spectre\ and \qsanndra\ \citep{qsanndra}, predict emission peaks closest to $\SI{1215.67}{\angstrom}$.} 
    \label{fig:ULASJ1120+0641_comp}
\end{figure}

==> captions/ULASJ1120+0641_wing.tex <==
\begin{figure}
	\includegraphics[width=\columnwidth]{figures/ULASj1120+0641_damping_wing_tight.png}
    \caption{This is an example figure. Captions appear below each figure.
	Give enough detail for the reader to understand what they're looking at,
	but leave detailed discussion to the main body of the text.}
    \label{fig:ULASJ1120+0641_wing}
\end{figure}


==> captions/ULASJ1342+0928.tex <==
\begin{figure*}
	\includegraphics[width=\textwidth]{figures/ULASJ1342+0928_tight.png}
    \caption{The observed spectrum of ULAS J1342+0928 ($z=7.54$) in grey overlaid with its smoothed continuum estimate in red and our prediction of its underlying intrinsic continuum in blue accompanied by 1-sigma (68\%) and 2-sigma (95\%) confidence intervals.}
    \label{fig:ULASJ1342+0928}
\end{figure*}

==> captions/ULASJ1342+0928_comp.tex <==
\begin{figure}
	\includegraphics[width=\columnwidth]{figures/ULASJ1342+0928_comp_tight_rev1.png}
    \caption{\spectre's prediction of ULAS J1342+0928's intrinsic blue-side spectrum compared with previous work by \citet{qsanndra}, \citet{daviesPCA},  \citet{greigLya}, and \citet{J1342}. The neural network models, \spectre\ and \qsanndra\ \citep{qsanndra}, predict a \lya\ peak closest to $\SI{1215.67}{\angstrom}$. }
    \label{fig:ULASJ1342+0928_comp}
\end{figure}

==> captions/ULASJ1342+0928_wing.tex <==
\begin{figure}
	\includegraphics[width=\columnwidth]{figures/ULASJ1342+0928_damping_wing_tight.png}
    \caption{This is an example figure. Captions appear below each figure.
	Give enough detail for the reader to understand what they're looking at,
	but leave detailed discussion to the main body of the text.}
    \label{fig:ULASJ1342+0928_wing}
\end{figure}

==> captions/autoregressive_transform.tex <==
\begin{figure}
	\includegraphics[width=\columnwidth]{figures/AutoregressiveTransform-rev2.png}
    \caption{Caption.}
    \label{fig:autoregressive_transform}
\end{figure}

==> captions/coupling_transform.tex <==
\begin{figure}
	\includegraphics[width=\columnwidth]{figures/CouplingTransform-rev2.png}
    \caption{Caption.}
    \label{fig:coupling_transform}
\end{figure}

==> captions/epca_bias_error.tex <==
\begin{figure}
	\includegraphics[width=\columnwidth]{figures/epca_bias_error_tight.png}
    \caption{}
    \label{fig:epca_bias_error}
\end{figure}

==> captions/neutral_fraction_comp.tex <==
\begin{figure}
	\includegraphics[width=\columnwidth]{figures/neutral_fraction_comp_tight_rev3.png}
    \caption{A comparison of our estimates of the volume-averaged neutral fraction of hydrogen for J1120+0641 ($z=7.09$) and J1342+0928 ($z=7.54$) to all previous approaches in the literature. Note that each approach employs a different damping wing model (and some employ full hydrodynamical models of the IGM) which complicates direct comparison. We attempt to remedy this by using the mean continua prediction of each previous approach to compute the neutral fraction of hydrogen with a single damping wing model (see Fig.~\ref{fig:neutral_fraction_comp_same_model}).}
    \label{fig:neutral_fraction_comp}
\end{figure}


==> captions/neutral_fraction_comp_same_model.tex <==
\begin{figure}
	\includegraphics[width=\columnwidth]{figures/neutral_fraction_comp_dw_model_no_err_tight.png}
    \caption{Neutral fractions for ULAS J1120+0641 and ULAS J1342+0928 computed from the mean intrinsic continua prediction of all previous approaches and a single damping wing model \citep{dampingWing}. Error bars are omitted since only mean continuum predictions are used. We note that all neutral fractions for J1342+0928 decrease using the \citealt{dampingWing} model. Compare to Fig.~\ref{fig:neutral_fraction_comp}.}
    \label{fig:neutral_fraction_comp_same_model}
\end{figure}

==> captions/preprocessing.tex <==
\begin{figure}
	\includegraphics[width=\columnwidth]{figures/preprocessing_tight.png}
    \caption{An example of a smoothed spectrum from our dataset overlayed on the raw flux observed from its quasar. We normalize the flux to unity at $\SI{1290}{\angstrom}$.}
    \label{fig:preprocessing}
\end{figure}

==> captions/random_inference_1.tex <==
\begin{figure}
	\includegraphics[width=\columnwidth]{figures/random_inference_tight1.png}
    \caption{This is an example figure. Captions appear below each figure.
	Give enough detail for the reader to understand what they're looking at,
	but leave detailed discussion to the main body of the text.}
    \label{fig:random_inference_1}
\end{figure}

==> captions/sdss_inference.tex <==
\begin{figure}
	\includegraphics[width=\columnwidth]{figures/random_inference_ext_sdss_tight_rev1.png}
    \caption{To infer the blue-side continuum, \spectre\ samples one thousand predictions of plausible blue-side continua conditional on the red-side. The assumed truth, shown in red, is the smoothed continua estimation from our preprocessing scheme, and the raw flux is shown in grey.}
    \label{fig:sdss_inference}
\end{figure}

==> captions/sdss_inference_no_red.tex <==
\begin{figure}
	\includegraphics[width=\columnwidth]{figures/random_inference_ext_sdss_no_red_tight.png}
    \caption{This is an example figure. Captions appear below each figure.
	Give enough detail for the reader to understand what they're looking at,
	but leave detailed discussion to the main body of the text.}
    \label{fig:sdss_inference_no_red}
\end{figure}

==> captions/tsne_train.tex <==
\begin{figure*}
	\includegraphics[width=\textwidth]{figures/tsne_train_tight.png}
    \caption{Two-dimensional representations of blue-side spectra from the training set and their associated \spectre\ predictions. We perform the dimensionality reduction using t-Distributed Stochastic Neighbor Embedding (t-SNE) with a variety of choices for the perplexity hyperparameter and find both distributions consistently overlap. Importantly, we show our predictions accurately sample from the training distribution.}
    \label{fig:tsne_train}
\end{figure*}


==> captions/tsne_valid.tex <==
\begin{figure*}
	\includegraphics[width=\textwidth]{figures/tsne_valid_tight.png}
    \caption{Two-dimensional embeddings of blue-side spectra from the validation set and their associated \spectre\ predictions. Embeddings were produced via t-Distributed Stochastic Neighbor Embedding (t-SNE) and we display the results for a series of perplexity choices. We find both distributions consistently overlap.}
    \label{fig:tsne_valid}
\end{figure*}
